Graded unitarity constraints on simply-laced affine Kac--Moody algebras

We investigate constraints imposed by four-dimensional unitarity (recently formalised as graded unitarity) on possible simply-laced affine Kac--Moody vertex algebras arising from four dimensions via the SCFT/VOA correspondence. Under the assumption that the $\mathfrak{R}$-filtration is weight-based with respect to the currents and the Casimir operators, with appropriately shifted $R$-charge assignments for the latter, we demonstrate that all values of the level other than a discrete set are incompatible with four-dimensional unitarity. This set includes all the boundary admissible affine vertex algebras, those corresponding to rank-one Kodaira SCFTs, as well as certain non-admissible families conjecturally associated with specific $D^b_q(\mathfrak{g})$ Argyres--Douglas theories. Specialising to $\mathfrak{sl}_N$ with $N$ prime, we find a stronger result: under the same $\mathfrak{R}$-filtration assumption, four-dimensional unitarity rules out all levels except the boundary admissible $k = k_{N,q}$, which are precisely those corresponding to the $D_q^N(\mathfrak{sl}_N)$ Argyres--Douglas theories.

==> topmatter.tex <==
%!TEX Root = ./main.tex

\RequirePackage{pdf14}
\RequirePackage{fix-cm}
\usepackage{./aux/jheppub}
\usepackage{longtable}
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{verbatim}
\usepackage{amsmath,amssymb,amsfonts,amsthm,amscd}
\usepackage{mathtools}
\usepackage{bm} %boldmath = \bm
\usepackage{bbm} %\mathbbm = doublestruck math for upper, lower, numbers, \mathbbmss=sans serif, \mathbbmtt=typewriter\
\usepackage{mathrsfs} %caligraphic
\usepackage{lscape} 
\usepackage{subcaption} 
%\usepackage[cal=boondox]{mathalfa} %lowercase \mathcal 
\usepackage{cancel}
\usepackage{enumitem}
\usepackage{tcolorbox}
\usepackage{multirow} % multiple row elements in a table
\usepackage{colortbl} % colored rows and columns in tables
\usepackage{array,hhline,multirow}
\usepackage{floatrow}
% \usepackage[margin=1in]{geometry}
% \usepackage{geometry}\geometry{margin=1in}
\newcommand{\cmark}{\text{\ding{51}}}%check mark
\newcommand{\xmark}{\text{\ding{55}}}%x mark
\usepackage[export]{adjustbox}
% \usepackage{ulem}
\usepackage{rotating} % rotate text
\usepackage[parfill]{parskip}
%FONTS AND MATH
\allowdisplaybreaks[2]  %allow page breaks in multi-line eqns, [1]=as little as poss; ... [4]=most permissive
\usepackage{pifont,dsfont}% http://ctan.org/pkg/pifont
\usepackage{array,setspace,mathrsfs,yfonts,dsfont,amscd,euscript}
\usepackage{relsize,suffix,mathtools,cancel,bm,bbm}


%TIKZ
\usepackage{graphicx,tikz}
\usepackage[framemethod=TikZ]{mdframed} % fancy boxes
\usepackage{tikz-cd} %for complicated commutative diagrams
\usepackage{tikz}
\usetikzlibrary{positioning}
\usepackage[table]{xcolor}

%COLORS
\usepackage{xcolor}
\def\red#1{{\color{red}{#1}}}
\def\blue#1{{\color{blue}{#1}}}
\def\green#1{{\color{black!30!green}{#1}}}
\def\blgr#1{{\color{black!15!blue!60!green}{#1}}}
\def\purple#1{{\color{purple}{#1}}}
\def\yellow#1{{\color{black!25!yellow!70!red}{#1}}}
\def\grey#1{{\color{black!40}{#1}}}
\definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
\definecolor{coolblack}{rgb}{0.0, 0.18, 0.39}
\definecolor{gold(web)(golden)}{rgb}{1.0, 0.84, 0.0}
\definecolor{deepcarmine}{rgb}{0.66, 0.13, 0.24}
\definecolor{knownSCFT}{RGB}{232,242,248}
\definecolor{newSCFT}{RGB}{232,245,235}
\definecolor{knownSCFTtext}{RGB}{40,100,140}
\definecolor{conjecturedSCFTtext}{RGB}{35,105,65}
\def\red#1{{\color{deepcarmine}{#1}}}
\def\green#1{{\color{green!70!black}{#1}}}
\def\Fgreen#1{{\color{ForestGreen}{#1}}}
\def\blue#1{{\color{blue}{#1}}}
\def\cblack#1{{\color{coolblack}{#1}}}
\def\bred#1{{\color{BrickRed}{#1}}}
\def\XSb{{\bar\cS}}
\def\bu{{\boldsymbol u}}
\def\XS{\mathfrak{S}}
\def\XSb{\bar{\XS}}
\def\H{\mathbb{H}}
\def\hTE{\hat{\CT}_{E_6,2}}
\def\tTE{\widetilde{\CT}_{E_6,2}}
\def\hTG{\hat{\CT}_{D_4,3}}
\def\hTA{\hat{\CT}_{A_2,4}}
\def\ccr{\cellcolor{red!15}}
\def\ccg{\cellcolor{green!15}} 

\newcommand{\Mc}{M(0,0;c)}
\newcommand{\Vc}{V(0,0;c)}
\newcommand{\Mhwc}{M(h,w;c)}
\newcommand{\Lvac}{$L_{-1}|0,0\rangle$ }
\newcommand{\Wvac}{$W_{-1}|0,0\rangle$ }
\newcommand{\Np}{$|\mathcal{N}_+\rangle$ }
\newcommand{\Nm}{$|\mathcal{N}_-\rangle$ }
\newcommand{\N}{$|\mathcal{N}\rangle$ }
\newcommand{\chip}{$|\chi_+\rangle$ }
\newcommand{\chim}{$|\chi_-\rangle$ }
\newcommand{\bV}{\mathbb{V}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mfR}{\mathfrak{R}}

\newcommand{\gf}{\mathfrak{g}}
\newcommand{\hf}{\mathfrak{h}}
\newcommand{\slf}{\mathfrak{sl}}
\newcommand{\sof}{\mathfrak{so}}
\newcommand{\spf}{\mathfrak{sp}}
\newcommand{\esixf}{\mathfrak{e}_6}
\newcommand{\esevenf}{\mathfrak{e}_7}
\newcommand{\eeightf}{\mathfrak{e}_8}

\newtheorem*{remark}{Remark}

\setcounter{tocdepth}{2}
